Causal Machine Learning for Healthcare and Precision Medicine

Causal machine learning (CML) has experienced increasing popularity in healthcare. Beyond the inherent capabilities of adding domain knowledge into learning systems, CML provides a complete toolset for investigating how a system would react to an intervention (e.g.\ outcome given a treatment). Quantifying effects of interventions allows actionable decisions to be made whilst maintaining robustness in the presence of confounders. Here, we explore how causal inference can be incorporated into different aspects of clinical decision support (CDS) systems by using recent advances in machine learning. Throughout this paper, we use Alzheimer's disease (AD) to create examples for illustrating how CML can be advantageous in clinical scenarios. Furthermore, we discuss important challenges present in healthcare applications such as processing high-dimensional and unstructured data, generalisation to out-of-distribution samples, and temporal relationships, that despite the great effort from the research community remain to be solved. Finally, we review lines of research within causal representation learning, causal discovery and causal reasoning which offer the potential towards addressing the aforementioned challenges.

==> same.tex <==

\section{Introduction}
\label{sec:intro}

Considerable progress has been made in predictive systems for medical imaging following the advent of powerful machine learning (ML) approaches such as deep learning \citep{litjens2017survey}. In healthcare, clinical decision support (CDS) tools make predictions for tasks such as detection, classification and/or segmentation from electronic health records (EHR) data such as medical images, clinical free-text notes, blood tests, and genetic data. These systems are usually trained with supervised learning techniques. That is, how observing a variable will change the belief that another variable has a given value? However, most CDS systems powered by ML techniques learn only associations between variables in the data, without distinguishing between causal relationships and (spurious) correlations. 

CDS systems targeted at personalized / precision medicine need to answer complex queries about how individuals would respond to interventions. A causal system modeling Alzheimer's disease, for instance, should be able to \emph{quantify} the effect of treating with a given drug in the final outcome, e.g.\ scores on a cognitive test. Even with the appropriate data and perfect performance, current ML systems would predict only the appropriate treatment based on previous correlations in data which may not represent actionable information. Such systems need causal inference (CI) in order to make individualized treatment effect predictions \citep{Bica2021}, allowing \emph{actionable} decision making (as detailed in Section \ref{sec:causal_healthcare}). Actionable predictive information about the effect of interventions will allow decision-makers to act based on a comparison between different scenarios (\textit{e.g.}\ outcome for treated or not treated) for a given patient. In other words, \textit{actionable} information empower the user to transition to the desirable side of the decision boundary. On the other hand, a single prediction (\textit{e.g.}\ outcome given a treatment) from traditional ML will purely reproduce the observational data patterns.

However, a major upstream challenge in healthcare is how to acquire the information needed to causally reason about treatments and outcomes. Modern healthcare data is multimodal, high-dimensional and often unstructured. Information from medical images, genomics, clinical assessments and demographics need to be taken into account for making predictions. In addition, many diseases diminish patient health during years. Therefore, the temporal aspects need to be taken into account. Finally, how can we make sure that these prediction will be generalisable across environments (different hospitals, cities or countries)?

Interestingly, the connection between causal inference and machine learning helps alleviate these challenges. ML allows causal models to process high-dimensional and unstructured data with complex (non-linear functions modelled by neural networks) relations between variables. CI adds an extra layer of understanding about a system with expert knowledge, which improves information merging from multimodal data, generalisation, and explainability of current ML systems.

The \emph{causal machine learning} (CML) literature proposes several ideas for the aforementioned challenges when using observational data. Here, we categorize CML into three classes of methods:
\begin{enumerate*}[label=(\roman*)]
    \item \textit{Causal Representation Learning} -- given high-dimensional data, learn to extract low-dimensional informative (causal) variables and their causal relations;
    \item \textit{Causal Discovery} -- given causal variables, learn the causal relationships between them;
    \item \textit{Causal Reasoning} -- given the causal variables and their relationship, analyse how a system will react to interventions.
\end{enumerate*}
We illustrate these ideas on Fig.\ \ref{fig:taxonomy} and further review representative methods for each of the categories and explain how they can be used in the healthcare context throughout the paper.

In this paper, we discuss how CML can improve personalized decision making in healthcare as well as helping mitigating pressing challenges in decision support systems. In particular, we 
\begin{enumerate*}[label=(\roman*)]
    \item present the concept of causality and causal models;
    \item show how they can be useful in healthcare;
    \item discuss pressing challenges, and
    \item review potential ideas from CML.
\end{enumerate*}


\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/taxonomy.pdf}
    \caption{Taxonomy of causal machine learning in healthcare. Healthcare data is multimodal, unstructured and high-dimensional. The ideas within \textit{causal machine learning} can be further divided into causal representation learning, causal discovery and causal reasoning.}
    \label{fig:taxonomy}
\end{figure}


\section{What is causality?}
We use a broad definition of causality: if $A$ is a cause and $B$ is an effect, then $B$ relies on $A$ for its value. As causal relations are directional, the reverse is not true, $A$ does not rely on $B$ for its value. The notion of \emph{causality} thus enables analysis of how a system would respond to an \emph{intervention}.

To illustrate, questions such as ``How will this disease progress if I give the patient treatment X?'' or ``Would this patient still have had outcome Z if they had been treated with treatment Y?'' require methods from causality to understand how an intervention would affect a specific individual. In a clinical environment, a causal reasoning can be useful for deciding which treatment will result in the best outcome. For instance, in a Alzheimer's patient scenario, causality can answer queries such as ``Would drug $A$ or drug $B$ improve the patient's probability of being cognitively normal after 5 years?''.
Ideally, we would compare the outcomes of alternative treatments in historical data. A \emph{fundamental problem of causal inference} \citep{10.2307/2289064}, however, states that for each unit (i.e. patient) we can observe either the result of treatment A or B, but never both at the same time. The reason is that after we have chosen to treat a patient, we cannot go back in time and undo the treatment. These queries that entertain hypothetical scenarios about individuals are called \emph{potential outcomes}. Thus, we can observe only one of the potential consequences of an action; the unobserved quantity becomes a \textit{counterfactual}. Causality's mathematical formalism pioneered by Judea Pearl \citep{pearl_2009} and Donald Rubin \citep{Imbens2015Causal}  allows these more challenging queries to be answered.

Most machine learning approaches are not (currently) able to identify cause and effect, because causal inference is fundamentally impossible to achieve without making assumptions \citep{pearl_2009,peters2017elements}. Several of these assumptions can be satisfied through study design or external contextual knowledge, but none can be discovered solely from observational data.


The rest of this section will introduce the reader to two ways of defining and reasoning about causal relationships with structural causal models in Sec.\ \ref{sec:scms}, potential outcomes in Sec.\ \ref{sec:potential_outcomes} and an introduction determining causal relationships including the use of randomized controlled trials in Sec.\ \ref{sec:randomized_control_trial}.


\subsection{Structural Causal Models}
\label{sec:scms}

The mathematical formalism around the so called \textit{do-calculus} and \emph{structural causal models} (SCMs) pioneered by the Turing Award winner Judea Pearl \citep{pearl_2009} has allowed a different graphical `domain knowledge-driven' perspective to reasoning with data. This framework can model the data generation process and include assumptions about a given problem. An intuitive and historical description of causality can be found in \citet{Pearl_why}'s recent book \emph{The Book of Why}. 

A SCM $\mathfrak{G} := (\mathbf{S},P_{\boldsymbol{N}})$ consists of a collection $\mathbf{S} = (f_1,....,f_K)$  of structural assignments (called mechanisms)
\begin{equation}
    X_k := f_k(\mathbf{PA}_k,N_k),
\end{equation}
where $\mathbf{PA}_k$ is the set of parents of $X_k$ (its direct causes) and $N_k$ is noise variable for modeling uncertainty. $\boldsymbol{N} = \{N_1,N_2,...,N_d\}$ is also referred to as \emph{exogenous} noise because it represents variables that were not taken into account by the causal model, as opposed to the \emph{endogenous} variables  $\boldsymbol{X} = \{X_1,X_2,...,X_d\}$ which are considered known or at least by design that they should be considered. This model can be defined as a direct acyclic graph (DAG) where the nodes are the causal variables and the edges are the mechanisms.

It is important to note that the causal mechanisms are representations of physical mechanisms that are present in the real world. Therefore, the principle of \emph{independent causal mechanisms} (ICM) is valid for these models. The principle states that the causal generative process of a system’s variables is composed of autonomous modules that do not inform or influence each other \citep{peters2017elements,scholkopf2021toward}. Therefore, exogenous variables $\boldsymbol{N}$ are mutually independent with the following joint distribution $P(\boldsymbol{N}) = \prod_{k=1}^{d} P(N_k)$. Moreover, the joint distribution over the endogenous variables $\boldsymbol{X}$ can be factorised as a product of independent conditional mechanisms
\begin{equation}
    P_{\mathfrak{G}}(X_1,X_2,..,X_K)=\prod_{k=1}^{K} P_{\mathfrak{G}}\left(X_{k} \mid \mathbf{PA}_{k}\right) .
\end{equation}

The causal framework, however, allows us to go beyond
\begin{enumerate*}[label=(\roman*)]
    \item associative predictions, answering
    \item interventional and
    \item counterfactual
\end{enumerate*}
queries. These three tasks are also known as Pearl's \textit{causal hierarchy} \citep{Pearl_why}. The \emph{do-calculus} introduces the notation $do(A)$, to denote a system where we have \emph{intervened} to fix the value of $A$. This allows us to sample from an interventional distribution $P^{\mathfrak{G};do(...)}_{\boldsymbol{X}}$.   The main difference between interventional and observational distribution $P^{\mathfrak{G}}_{\boldsymbol{X}}$ is that the causal structure forces that only the descendants of the variable intervened upon will be modified by a given action. 

\subsection{Potential Outcomes}
\label{sec:potential_outcomes}
An alternative approach to causal inference is the \emph{potential outcomes} framework proposed by  \citet{rubin2005causal}. In this framework, a response variable $Y$ is used to measure the effect of some cause or treatment for a patient, $i$. The value of $Y$ may be affected by the treatment assigned to $i$. To enable the treatment effect to be modelled, we need to represent the response with \emph{two} variables $Y_{i}^{(0)}$ and $Y_{i}^{(1)}$, untreated and treated respectively. This then allows the to represent the  effect of the treatment on $i$ as $Y_{i}^{(1)} - Y_{i}^{(0)}$.
     
As a patient may \emph{potentially} be untreated or treated, we refer to $Y_{i}^{(0)}$ and $Y_{i}^{(1)}$ as \emph{potential outcomes}. It is, however, impossible to observe both simultaneously, which is the \emph{Fundamental Problem of Causal Inference} \citep{10.2307/2289064}. This does not mean that causal inference itself is impossible, but it does brings challenges \citep{Imbens2015Causal}. Causal reasoning in the potential outcome frameworks depends on obtaining an estimate for the joint probability distribution, $P(Y^{(0)}, Y^{(1)})$.

Both SCM and potential outcomes approaches have useful applications, and are used where appropriate throughout this report. We note that single world intervention graphs \citep{richardson2013single} have been proposed as a way to unify them.

\subsection{Determining Cause and Effect} 
\label{sec:randomized_control_trial}

Determining causal relationships often requires carefully designed experiments. There is a limit to how much can be learned using purely observational data such as Electronic Health Records.

The effects of causes can be determined through prospective experiments to observe an effect $E$ after a cause $C$ is tried or withheld, keeping constant all other possible factors. It is hard and in most cases impossible to control for all possible confounders of $C$ and $E$. The gold standard for discovering a true causal effect is by performing a randomized controlled trial (RCT), where tthe choice of $C$ is randomized, removing confounding.

For example, by giving a COVID-19 vaccine to a randomized group of people and placebo to another in an interventional study, we can measure the effect of the vaccine, eliminating any bias that may have arisen in an observational study due to other confounding variables, such as lifestyle factors, that influence both the choice of using the vaccine and the impact of COVID-19.


Note that the conditional probability $P(E \mid C)$ of observing $E$ after observing $C$ can be different from the interventional probability $P(E \mid do(C))$ of observing $E$ after doing $C$. In RCTs, the ‘do’ is guaranteed and unconditioned, while with observational data such as Electronic Health Records, it is not due to the presence of confounders.

Determining the causes of effects requires hypotheses and experimentation where interventions are made and studied to determine the necessary and sufficient conditions for a an effect to occur. In medicine, this is the field of aetiology.

\section{Why should we consider a causal framework in Healthcare?}
\label{sec:causal_healthcare}

Causal inference has made several contributions over the last few decades to fields such as social sciences, econometrics, epidemiology, and aetiology  \citep{pearl_2009,Imbens2015Causal}, and it has recently spread to other healthcare areas such as medical imaging \citep{castro2020causality,Pawlowski,Reinhold2021} and pharmacology \citep{Bica2021}. In this section, we will elaborate on how causality can be used for improving medical decision making. 

Even though data from electronic health records (EHRs), for example, are usually observational, they have already been successfully leveraged in several machine learning applications \citep{PICCIALLI2021111}, such as modeling disease progression \citep{Lim2018}, predicting disease deterioration \citep{prediction_kidney_nature}, and discovering risk factors \citep{McCauley2016}, as well as predicting treatment responses \citep{Athreya_1482}. We have algorithms with superhuman performance in tasks such as segmentation \citep{isensee2021nnu}, detection, classification \citep{korot2021code} and regression of anatomies and/or pathologies from images and other entries of electronic health records. However, predicting a disease with almost perfect accuracy for a given patient is still not what precision medicine is trying to achieve \citep{Wilkinson2020}. Building machine learning methods to extract \emph{actionable} information from observational patient data involves \emph{causal inference}, which goes beyond standard supervised learning methods for prediction as detailed below.

In order to make actionable decisions at the patient level, one needs to identify the treatment effect. The treatment effect is the \emph{difference} between two potential outcomes: the \emph{factual} outcome and the \emph{counterfactual} outcome.  For actionable predictions, we need algorithms that learn how to reason about hypothetical scenarios where different actions would have been taken. Creating, therefore, a decision boundary that can be navigated in order to improve patient outcome. There is recent evidence that humans use counterfactual reasoning for making causal judgements \citep{Gerstenberg2021csm}, solidifying this reasoning hypothesis.

This is what makes the problem of inferring treatment effect fundamentally different from standard supervised learning \citep{Bica2021} as defined by the potential outcome framework \citep{rubin2005causal,Imbens2015Causal}. When using observational datasets, by definition, we never observe the counterfactual outcome. Therefore, the best treatment for an individual - the main goal of precision medicine \citep{zhang2018learning} - can only be identified with a model that is capable of causal reasoning as will be detailed in section \ref{sec:precision_medicine}.

 
\subsection{Running Example} 

We now illustrate the notion of causal machine learning for healthcare with an example within \textit{Alzheimer's disease} (AD). A recent attempt to understand Alzheimer's from a causal perspective takes into account many biomarkers and uses domain knowledge (as opposed to RCTs) for deriving ground truth causal relationships. In this section, we present a simpler view with only three variables: chronological\footnote{Age can otherwise be measured in biological terms using, for instance, DNA methylation \citep{Horvath2013DNAm}.} age, magnetic resonance (MR) image of the brain, Alzheimer's diagnosis. We are particularly interested in MRI images because analysing the relationship of high-dimensional measures, such as an MRI image and diagnosis, is a task that can be more easily handled with machine learning techniques, the main focus of this paper.

AD is associated with brain atrophy \citep{Karas2004NeuroImage,Qian2019}, and it is well-known that volumetric changes in grey matter occur during ageing \citep{Sullivan1995Neurobiology,Good2001Morphometric}. At the same time, Alzheimer's disease is a cognitive decline that generally appears later in life \citep{Jack2015JAMA}. Time does not depend on any biological variable, therefore chronological age cannot be caused by AD nor any change on brain morphology. In this scenario, we can assume that age is a confounder of brain morphology, measured by the MR image, and Alzheimer's disease. 

We consider that Alzheimer's disease causes the symptom brain morphology change, following \citet{Richens2021nature}. The causal direction between brain morphology and Alzheimer's by argument that a high-dimensional variable such as the MRI image is caused by the factors the generated it, this modelling choice has been previously used in the causality literature \citep{Scholkopf2012anticausal, kilbertus2018generalization,Deml2021Anti}.

To illustrated the effect of having age as a confounder of brain morphology and Alzheimer's disease, we use a conditional generative model from \citet{xia2019learning}. We synthesise images of a patient at different ages and with different Alzheimer's disease status as depicted in Fig\ \ref{fig:alzheimers_scm}. In particular, we control for one variable while intervening on the other. That is, we synthesise images based on patient that is cognitively normal (CN) at age 64 years old. We fix the Alzheimer's status at CN and increase the age of 3 years for 3 steps, resulting in images of the same CN patient at ages 64, 67, 70, 73. At the same time, we synthesise images with different Alzheimer's status by fixing the at 64 and changing the Alzheimer's status to mild cognitive impairment (MCI) and to full Alzheimer's disease (AD). 

By observing qualitatively the difference between the baseline and synthesised images, one might arrive to the conclusion that ageing and Alzheimer's disease have similar effects on the brain. That is, both variables change the volume of brain when intervened on independently. See \citet{xia2019learning} for more quantitative results. The synthesised images of the Alzheimer's seems to have a stronger effect, but they are nevertheless similar. This example illustrates how the effect of \textit{confounding bias}.

Throughout the paper, we will further add variables and causal links into the problem to illustrate how healthcare problems can become more complex and how a causal approach might mitigate some of the main challenges. In particular, we will build on top of this example by explaining some consequences of causal modelling for dealing with high-dimensional and unstructured data, generalization and temporal information. 


\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/alzheimers_scm.png}
    \caption{Causal graph (\textit{left}) and illustration of how the brain changes in MRI images and intervening on ``Age" or ``Alzheimer's" status. The images are axial slices of a brain MRI. The middle image used as a baseline is from a patient aged 64 years old and classified an cognitively normal (CN) within the Alzheimer’s Disease Neuroimaging Initiative (ADNI) database. All other images are synthesised with a conditional generative model \citep{xia2019learning}. The images with grey background are difference images obtained by subtracting the synthesised image from the baseline. The upper sequence of images are generated by fixing Alzheimer's status at CN and increasing age by 3 years. The bottom images are generated by fixing the age at 64 and increasing Alzheimer's status to MCI and AD, as discussed in the main text.}
    \label{fig:alzheimers_scm}
\end{figure}



\subsection{Modeling the Data Generation Process}
\label{sec:data_gen_process}


In the Alzheimer's disease setting above, a classifier naively trained for performing diagnosis from MRI images of the brain might focus on the brain's atrophy alone. Due to the confounding bias issue, this classifier results in a performance drop across different age groups, leading to potentially incorrect diagnosis. To illustrated this point, we report the results of a convolutional neural network (CNN) classifier trained and tested on the ADNI dataset following the same setting as \citet{xia2022adversarial}\footnote{Even thought we replicate results from \citet{xia2022adversarial}, this work does not constitute an extension of the original paper. We only use \citet{xia2022adversarial} as an example that illustrates how causality might impact standard machine learning.}. We show the confounding bias phenomenon using the stratified diagnosis accuracy on the test set in Tab.\ \ref{tab:alzheimer_class}. As expected, healthy older patients (80-90 years old interval) are less accurately predicted because ageing itself causes the brain to have Alzheimer's-like patterns.

\begin{table}[]
\caption{Illustration of how a naively trained classifier fails when the data generation process and causal structure are not identified. We show the classification accuracy on the test set of a naively trained neural network. The results are stratified by age as well as by Alzheimer's status. We highlight that the {\color{r2} worse performance} group is with older cognitively normal patients due to the confounding bias described in the main text. These results were replicated from \citet{xia2022adversarial}.}
\label{tab:alzheimer_class}
\begin{center}
\begin{tabular}{cclll}
\hline
\multicolumn{2}{c}{Age Range}                             & 60-70 & 70-80 & 80-90                       \\ \hline
                           & Cognitively Normal & 85.2  & 91.5  & {\color{r2} 70.7} \\ \cline{2-5} 
\multirow{-2}{*}{Accuracy} &  Alzheimer's& 90.5  & 91.2  & {\color{b2} 97.1} \\ \hline
\end{tabular}
\end{center}
\end{table}
%\multicolumn{1}{c|}{ }
The Alzheimer's diagnosis example illustrates the importance of considering causal relationships in a machine learning scenario. Namely, causality brings the ability to model and identify types and sources of bias\footnote{we refer to \url{https://catalogofbias.org/biases} for a catalogue of bias types}. To correctly identify which variables to control for (as means to mitigate confounding bias), causal diagrams \citep{pearl_2009} offer direct means of visual exploration and consequently explanation \citep{Brookhart2010,Lederer2019Annals}.

\citet{castro2020causality}, for example, details how understanding the causal generating process can be useful in medical imaging. By creating a graph representing the variables of a particular problem and what is their causal relationship , one can model \emph{domain shifts} such as population shift (different cohorts), acquisition shift (different sites or scanners) and annotations shift (different annotators) and data scarcity (imbalanced classes). 

%They also detail the difference in making predictions in two difference settings: causal - prediction effect from cause. For example,  classification of skin cancer in images when the ground truth is obtained with biopsy as illustrated in \ref{fig:causality_matters_graph} by the $Y_1$ variable prediction; anti-causal - predicting cause from effect. For example, segmentation of breast cancer from CT scans when ground truth is created by inspecting the image (masks are caused by the image) as illustrated in \ref{fig:causality_matters_graph} by the $Y_4$ variable prediction. %and its consequences for machine learning.

With this knowledge, one can devise the best strategies for mitigating the bias in the data and improving generalization. For example, if after modeling the data distribution, one realizes that there is an acquisition shift in their problem (e.g. training data was obtained with a specific MRI sequence but the model will be tested with a different sequence), one can design data augmentation strategies to increase robustness of the learned representation. The acquisition shift - e.g. different intensities due to different scanners - might be modeled according to the physics of the systems. Ultimately, creating a diagram of the data generation process helps rationalize/visualize which are the best strategies to solve the problem. Indeed, using augmented data based on the causal knowledge is the solution found in \citet{xia2022adversarial}. They reduce the bias issue by augmenting the training data with counterfactual images of a patient when intervened on age. That is, they synthesise images of a patient at different ages (while controlling for Alzheimer's status) so the classifier learns how differentiate the effects of ageing vs Alzheimer's disease in brain images.


\subsection{Treatment Effect and Precision Medicine}
\label{sec:precision_medicine}

Beyond diagnosis, a major challenge in healthcare is ascertaining whether a given treatment influences or determines an outcome. For a binary treatment decision, for instance, the aim is to estimate the \emph{average treatment effect} (ATE), $E[Y^{(1)} - Y^{(0)}]$ where $Y^{(1)}$ is the outcome given the treatment and $Y^{(0)}$ is the outcome without it (control). As it is impossible to observe both potential outcomes $Y^{(0)}$ and $Y_{i}^{(1)}$ for a given patient $i$, this is typically estimated using $E[Y|T=1] - E[Y|T=0]$, where $T$ is the treatment assignment. 

The treatment assignment and outcomes, however, both depend on the patient's condition in normal clinical conditions. This results in confounding, which is best mitigated by the use of a RCT \ref{sec:randomized_control_trial}. Performing a RCT as detailed in Sec.\ \ref{sec:randomized_control_trial}, however, is not always feasible, and causal inference techniques can be used to estimate the causal effect of treatment from observational data \citep{Meid2020}. A number of assumptions need to hold in order for the treatment effect to be identifiable from observational data, including: (conditional) exchangeability, positivity, and consistency \citep{Lesko2017}. Continuing the Alzheimer's example, \citet{Charpignon2021}, for instance, explore drug re-purposing by emulating a RCT with a target trial \citep{hernan2016using} and find indications that metformin (a drug classically used for diabetes) might prevent dementia.

Note that even if the treatment effect is estimated using data from a well-designed RCT, $E[Y|T=1] - \E[Y|T=0]$ is the \emph{average} treatment effect across the study population. However, there is evidence \citep{Bica2021} that for any given treatment, it is likely that only a small proportion of people will actually respond in a manner that resembles the ``average'' patient. \emph{Precision medicine} aims to determine the best treatment for an \emph{individual} \citep{Wilkinson2020}, rather than if it improves the average response in a population. In order to answer this question for a binary treatment decision, it is necessary to estimate $ \tau_i = Y_i(1) - Y_i(0)$ for a patient $i$ . This is known as the individualized treatment effect (ITE). As this estimation is performed using a conditional average, this is also referred to as the conditional average treatment effect (CATE).

%  \begin{align*}
%      E_X[\tau(x)] &= E_X[E[Y(1) - Y(0) \ | \ X = x]] && \mbox{(ATE)} \\
%      \tau_i &= Y_i(1) - Y_i(0) && \mbox{(ITE)} \\
%      \tau(x) &= E[Y(1) - Y(0) \ | \ X = x] && \mbox{(CATE)} \\
%  \end{align*}
 
A number of approaches have been proposed to learn this from observational data. Estimating treatment effect with double machine learning \citep{Chernozhukov2018-mt}. Another trend for estimating ITE are the meta-learners \citep{kunzel2019metalearners,curth2021nonparametric}, which are build on top of base supervised learning algorithms. While most approaches concentrate on estimating ITE using observational data, it is also possible to do so using data from an RCT \citep{Hoogland2021}. We show in Fig.\ \ref{fig:ite}

Some argue that the goal of precision medicine faces serious challenges, many of which cannot be addressed through algorithmic complexity, and call for collaboration between traditional methodologists and experts in medical machine learning \citep{Wilkinson2020}. One needs to distinguish between prediction (which only find associations in data) and intervention models because the latter is needed for actionable decision-making \citep{Prosperi2020}.

A long-term goal of precision medicine \citep{Bica2021} includes personalized risk assessment and prevention. Without a causal model to distinguish these questions from simpler prediction systems, interpretational mistakes will arise. In order to design more robust and effective machine learning methods for personalized treatment recommendations, it is vital that we gain a deeper theoretical understanding of the challenges and limitations of modeling multiple treatment options, combinations, and treatment dosages from observational data. 


\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/ite_ate_counterfactual.pdf}
    \caption{By using causal inference methods to estimate individualized treatment effects, we can understand which patients benefit from certain medication and which patients do not, thus enabling us to make personalized treatment recommendations.}
    \label{fig:ite}
\end{figure}

\section{Challenges}
\label{sec:learn_variables}

%Causal reasoning is mostly concerned with quantifying the effect of a change of variables on each other for a given causal model. In this setting, we usually consider that (or at least part of) the structural causal model (SCM defined in section \ref{sec:causal_models}) is \textbf{known}. Being able to apply interventions in specific variables of a model and observe their causal effect can be extremely useful for decision-making as detailed in section \ref{sec:healthcare}. It also allows for counterfactual reasoning, estimating what the outcome might had been had variables taken different values.

Using causal models for understanding a data generation process (Sec.\ \ref{sec:data_gen_process}) and quantifying causal effects (Sec.\ \ref{sec:precision_medicine}) is referred to as \emph{causal reasoning}. In this setting, one usually considers that the causal model is \emph{known} (at least partially). Being able to apply interventions in specific variables of a model and observe their causal effect can be extremely useful for medical decision-making as detailed in Sec.\ \ref{sec:causal_healthcare}. We refer the reader to \citet{Bica2021} for a comprehensive review on these methods.

Most healthcare problems, however, have challenges that are upstream of causal reasoning. In this section, we describe some pressing challenges from healthcare that can be mitigated with causal machine learning. We detail the importance of dealing with high-dimensional and multimodal data as well as with temporal information and discuss generalisation in out-of-distribution settings when learning from unstructured data. In Sec.\ \ref{sec:solutions} we review potential solutions from the causal machine learning literature for solving this problem.


%Causal inference addresses the problem of ascertaining causes and effects from data. Following the terminology of a recent book on causality \cite{peters2017elements}, the term causal inference comprises two somewhat complementary scenarios:
%\begin{enumerate}[label=(\roman*)]
%    \item \textit{causal discovery} which is concerned with inferring causal models from empirical data;
    %\item \textit{causal reasoning} which employs causal models for inferring about the expected observations (often, about their statistical properties).
%\end{enumerate}
%Both parts crucially depend on assumptions on the statistical properties entailed by hypothetical causal structures. The general idea is that causal structure (the model) is a concept that often remains invariant across changing background conditions \cite{peters2017elements} can be utilized for both causal reasoning and causal discovery. 


\subsection{High-Dimensional and Multimodal Healthcare Data}
\label{sec:dimension_modal}

Alzheimer's disease, as well as most major health issues such as diabetes and cancer, is a complex disorder. The disease has multiple causes arising from complex interaction between genetics and environmental factors. Indeed, recent attempts \citep{Shen2020Discovery,Uleman2020Alzheimer} to build a causal graphs for describing Alzheimer's disease take into account data derived from several data sources and modalities. For instance, information from the patients demographics, i.e. clinical, genetic and imaging exams, were used for constructing a causal diagram.

Another recent example \citep{Belyaeva2021} illustrates the importance of considering multimodal information in healthcare for drug repurposing. \citet{Belyaeva2021} discover potential drugs for the SARS-CoV-2 virus by identifying druggable protein targets, given the pressing challenges arising from the recent pandemic. In order to identify potential drug candidates for COVID-19, they integrated RNA-seq data from cells infected by SARS-CoV-2, RNA-seq data from the lungs of young and old individuals, protein–protein interaction data, drug–target data and data from the transcriptional drug screen Connectivity Map (CMap). %They further used a causal discovery method \citep{Wang2017Permutation} to understand which genes can be modulated by a drug. 

The two examples above illustrates that modern healthcare is multimodal. New ways of measuring biomarkers are increasingly more available, but merging this information is not trivial. The common information across modalities needs to be disentangled from the unique information within each modality. Information from different sources need to be transformed to a space where information can be combined. This is critical for developing CDS systems capable of integrating data images, text and genomics data.

At the same time, the availability of more variables might mean that some assumptions classically done in causal inference are more realistic. In particular, most methods consider the assumption of \emph{ignorability} \citep{Imbens2015Causal} or causal \emph{sufficiency} \citep{spirtes2000causation}, which implies no hidden (unobserved) confounders. In other words, given certain covariates, it is possible
to \emph{ignore} other covariates as if they were randomized. In practice, the assumption is often not true. However, observing more variables might reduce the probability of important variables to be hidden, making the ignorability assumption more plausible.

%and the need to obtain phenotyping information from these images (beyond their diagnostic and prognostic value) introduce different challenges to the high-dimensional variables involved. 
%In these cases, learning causal representations \citep{scholkopf2021toward} became an essential part for solving the problem. We discuss in Sec.\ \ref{sec:causal_representation_learning} some recent advances in the field and how they might be used in the imaging domain.

%That is the main reason why machine learning can have a impact on the causal inference formalism. Recent advances in representation learning (\cite{CHARTSIAS2019101535,Pawlowski,papamakarios2019normalizing}) will allow multimodal data to be transformed to a space where information can be combined. This is critical for developing CDS systems capable of integrating data images, text and genomics data. Disentangling representations from high-dimensional data is still a open research question and largely the topic of the RAEng project in itself.
%Firstly, the effects of some interventions are not even identifiable, we need to have knowledge about the causal structure of the problem for achieving such conclusions. This requires tools from \emph{causal discovery} \citep{Glymour2019frontiers}. Causal discovery is concerned with inferring causal models from empirical data.

%In addition,  Luckily, modern healthcare is highly multimodal and new technologies, such as wearable devices, for constantly monitoring patients are being created everyday. However, leveraging all available information is not straightforward due to valuable but unstructured data sources such as medical images, free text reports and genomics. The emergent field that aims at extracting high-level and causally structured features form high-dimensional variables is entitled \textit{causal representation learning} \citep{scholkopf2021toward}. We refer the reader to Fig.\ \ref{fig:taxonomy} for an illustration of a complete understanding the taxonomy of the causal machine learning framework.


\subsection{Temporal Data}

Using temporal information for inferring causation can be traced back to one of the first definitions of causality by \citet{Hume1904HUMECH}. Quoting Hume, ``we may define a cause to be an object followed by another, and where all the objects, similar to the first, are followed by objects similar to the second". A classical model of causality for time-series was developed by \citet{granger1969investigating}. \citeauthor{granger1969investigating} consider $X \rightarrow Y$ if past $X$ is predictive of future $Y$. Therefore, inferring causality from time series data is at the core of CML.

On the other hand, managing diseases, such as Alzheimer's disease and other neurodegenerative diseases, can be challenging due to heterogeneity of symptoms and their trajectory over time across the population. A pathology might evolve differently for patients with different covariates. For instance, it is well known that genetic factors contribute for different disease trajectories in Alzheimer's disease \citep{Mishra2018}. Using data-driven approaches for understanding and modelling the progression of diseases over time \citep{Oxtoby2017neurodegenerative} can be helpful. Early work used causal inference focused on neuroscience \citep{friston2003dynamic}, but using between temporal causal inference associated with machine learning for dealing with complex disease remains largely unexplored.

In addition, When one wishes to make treatment decisions in a longitudinal setting, causal inference methods need to model patient history and treatment timing \citep{soleimani2017treatmentresponse}. Estimating counterfactual trajectories under different treatment plans in the future is extremely important \citep{Bica2020Estimating}. CDS systems need to take into account the current health state of the patient and make predictions about the best treatments and potential outcomes. The knowledge of hypothetical future possibilities enables decision-makers to choose the sequence and timing of treatments that lead to the best patient outcome \citep{Bica2021}. 

%\sat{i think this example we should expand more.  It is important to discuss hat is an outcome? how this will be captured in an SCM what challenges remain, see also last comment in this section!}
%Fig. \ref{fig:time_series_prediction} illustrates an example of how a system can help in decision making for a breast cancer patient with multiple choices of treatment (chemotherapy and radiotherapy). The system needs to take into account the current health state of the patient and make predictions about outcomes such as the probability of survival after 5 years. On top of that, a causal model will be able to take complex multimodal data as inputs and apply interventions on treatment in order to help making decision towards the best patient outcome. As discussed, the machine learning model needs to be designed to take into account expert knowledge and the causal framework in order to estimate the counterfactual trajectories.

%Recent work \citep{prediction_kidney_nature,Lim2018, Bica2020Estimating, pmlr-v119-bica20a} has solved this problem with sequence-to-sequence models that leverage the increasing availability of patient observational data, as well as recent advances in representation learning, recurrent neural networks and domain adversarial training, to estimate treatment effects over time. Other approaches used Bayesian nonparametrics \citep{10.1093/biostatistics/kxw029,soleimani2017treatmentresponse} to estimate longitudinal treatment effects.

\subsection{Unstructured data and Out-of-Distribution Generalization}

The challenge of integrating different modalities and temporal information intensifies when unstructured data is used. Most of the causality theory has originally been developed in the contexts of epidemiology, econometrics, social sciences, and other fields wherein the variables of interest tend to be scalars \citep{pearl_2009,Imbens2015Causal}. In healthcare, however, the use of imaging exams and free-text reports poses significant challenges for consistently and robustly extracting meaningful information. Processing unstructured data is mostly tackled with machine learning, and \emph{generalization} is one of the biggest challenges for learning algorithms. 


As the use of machine learning in high impact domains becomes widespread, the importance of evaluating safety has increased. An important aspect of this is evaluating how robust a model is to changes in environment (or domain), which typically requires applying the model to multiple, independent datasets \citep{pmlr-v130-subbaswamy21a}. Since the cost of collecting such datasets is often prohibitive, causal inference argues that giving structure (which comes from expert knowledge) is required for increasing robustness in real life \citep{pearl_2009}.

In its most basic form, generalization is the ability to correctly categorize new samples that differ from those used for training \citep{bishop2006pattern}. However, when learning from data, the notion of generalization has many facets. Here, we are interested in a realistic setting where the test data distribution might be different from the distribution of the training data. This setting is often referred to \textit{out-of-distribution (OOD) generalization}. We wish to present a causal perspective \citep{Gong2016,Rojas2018jmlr,Meinshausen2018} on generalization which unifies many machine learning settings. 

We consider the view \citep{Scholkopf2012anticausal, kilbertus2018generalization,Deml2021Anti,rosenfeld2021the} that most prediction problems are in the anti-causal direction\footnote{We note that other important works \citep{Peters2016invariant,Arjovsky2019irm} consider prediction a causal task because prediction should copy a cognitive human process of generating labels given the data.}. That is, when making a prediction from a high-dimensional , unstructured variable $X$ (\emph{e.g.}\ brain image) one is usually interested in extracting and/or categorizing one of its true generating factors $Y$ (\emph{e.g.}\ gray matter volume). However, another (or many others) generating factor $W$ is often correlated with $Y$, which might cause the predictor to learn the relationship between $X$ and $W$ instead of the $Y = f(X)$. This is known as a shortcut \citep{Geirhos2020} due to the \textit{spurious correlation}. We also consider an environment variables $Env$ which controls the relationship between $Y$ and $W$. $Env$ is a confounder  $Y \leftarrow Env \rightarrow W$ and $X$ is caused by the two variables $Y \rightarrow X \leftarrow W$. This setting is illustrated in Fig.\ \ref{fig:generalization}.


\begin{figure}[h]
    \centering
    \includegraphics[width=.5\linewidth]{figures/generalization_fig.pdf}
    \caption{Reasoning about generalization with a causal graph.}
    \label{fig:generalization}
\end{figure}

The domain of $Env$ is define as a discrete set $\{1,2, \dots, e\}$. Then, the tuple $(\mathbf{x},\mathbf{y})^e$ is a set of samples from joint distribution over $P(X,Y \mid Env = e)$. Imagine a prediction problem where the goal is learn $f: Y \leftarrow X$. We can now describe several machine learning setting based on this causal perspective by comparing the data availability during train and test time. %as summarised in Tab.\ \ref{tab:causal_generalization}.


%\input{tables/generalization}


Classical \emph{supervised learning} (or empirical risk minimization (ERM) \citep{vapnik1999overview}) uses the strong assumption that the data from train and test sets are \emph{independent and identically distributed (i.i.d.)}, therefore we assign the same environment for both sets. \emph{Semi-supervised learning} is a case where part of the training samples are not paired. \emph{Continual (or Lifelong) learning} considers the case where data from different environments are added after training, and the challenges is to learn new environments without forgetting what has been initially learned. In \textit{domain adaptation}, only unpaired data of test environment is available during training. \textit{Domain generalization} aims at learning how to become invariant to changes of environment, such that a new (not in train data) environment can be used as test set. Enforcing \textit{fairness} is important when $W$ is a sensitive variable and the train set has $Y$ and $W$ spuriously\footnote{ We use the term \textit{spurious} for features that correlates but do not have a causal relationship between each other.} correlated due to a choice of environment. Finally, learning from \textit{imbalanced} datasets can be seen under this causal framework when a specific $Y = y$ have different number of samples because of the environment, but test environment might contain the same bias towards a specific value of $Y$.

\section{Ideas from Causal Machine Learning}
\label{sec:solutions}

Having discussed the utility of CML for healthcare and what are some of the pressing challenges, the final section of this paper introduce ideas and research directions in the literature. As mentioned in Sec.\ \ref{sec:intro}, we categorize CML into three classes of methods (to be defined in the respective sections)
\begin{enumerate*}[label=(\roman*)]
    \item Causal Representation Learning;
    \item Causal Discovery;
    \item Causal Reasoning.
\end{enumerate*}

\subsection{Causal Representations}
\label{sec:causal_representation_learning}

Representation learning \citep{6472238} refers to a \textit{compositional} view of machine learning. Instead of a mapping $f$ between input $\mathcal{X}$ and output $\mathcal{Y}$ domains denoted by $\mathcal{X} \xrightarrow[]{f} \mathcal{Y}$, we consider a representation $\mathcal{Z}$ that captures concepts about world ($\mathcal{X} \xrightarrow[]{E} \mathcal{Z} \xrightarrow[]{D} \mathcal{Y}$), with $f : E \circ D$. Where $E$ and $D$ are called here the ``encoder'' and the ``decoder''\footnote{We also use $D$ to refer to a classification or regression mapping, not only decoding a latent representation back to input domain.}. This notion is essential when considering learning and reasoning with real healthcare data. High-dimensional and unstructured data are not organized in units that can be directly used in our causal models. In most situations, the variable of interest is not, for instance, the image itself, but one of its generating factors. 

\emph{Causal} representation learning \citep{scholkopf2021toward} extends the notion of learning concepts about world to modelling the relationships between variables with causal models. In other words, the goal is to model the representation domain $\mathcal{Z}$ as an SCM as in Sec.\ \ref{sec:scms}. Causal representation learning builds on top of the \emph{disentangled} representation learning literature \citep{Higgins2017betaVAELB,kim2018disentangling,chen2016infogan,liu2021tutorial} towards stronger inductive bias. The idea is to reinforce a hierarchy of latent variables following the causal model, which in turn should follow the real data generation process.

\subsection{Causal Discovery}
\label{sec:causal_discovery}


Performing RCTs is very expensive and sometimes unethical or even impossible. For instance, to understand the impact of smoking in lung cancer, it would be necessary to force random individuals to smoke or not-smoke. Most real data are observational and discovering causal relationships between the variables is more challenging. Considering a setting where the causal variables are \textbf{known}, \textit{causal discovery} is the task of learning the direction causal relationships between the variables. In some settings, we have many inputs variables and the goal is to construct the graph structure that best describes the data generation process. 

There is extensive literature developed over the last 3 decades around discovering causal structures from observational data, as detailed in recent reviews of the subject \citep{peters2017elements,Glymour2019frontiers,Nogueira2021,vowels2021dya}. Most methods rely on assumptions about the functions classes (e.g. additive noise) and noise distributions (e.g. Gaussian) for finding the causal relations of given causal variables. 

Causal discovery is still an open area of research and some of the major challenges in discovering causal effects \cite{peters2017elements, Prosperi2020} from observational data are the inability to
\begin{enumerate*}[label=(\roman*)]
    \item identify all potential sources of bias (unobserved confounders); 
    \item select an appropriate functional form for all variables (model misspecification); and
    \item model temporal causal relationships.
\end{enumerate*}

%The bias reinforced by the knowledge structure from causal models should lead to mechanisms - functions/relations between variables - that are more robust and more generalizable. 


\subsection{Causal Reasoning}

It has been conjectured that humans internally build generative causal models for imagining approximate physical mechanisms through intuitive theories \citep{kilbertus2018generalization}. Similarly, the development of models that leverage the power of causal models around interventions would be useful. The causal models from Sec.\ \ref{sec:scms} and \ref{sec:potential_outcomes} can be formally manipulated for measuring the effects of interventions. Using causal model for quantifying the effect of interventions and pondering about the best decision is known as \textit{causal reasoning}.

Causal reasoning also refers to the ability to answer counterfactual queries such as``What would have happened if the patient had received another treatment?''. We elaborate at length on the benefits of counterfactuals in the healthcare context in Sec.\ \ref{sec:precision_medicine}. 

One of the key benefits of reasoning causally about a problem domain is transparency, by offering a clear and precise language to communicate assumptions about the collected data \citep{chou2021counterfactuals,rudin2019stop,castro2020causality} as detailed in Sec.\ \ref{sec:data_gen_process}. In a similar vein, models whose architecture mirrors an assumed causal graph can be desirable in applications where interpretability is important \citep{moraffah2020causal}.

The main challenges in causal reasoning with ML are around performing interventions with complex data representations and functions. The strategies for counterfactual prediction are simpler with scalar variables and linear functions. Interventions can have qualitatively distinct behaviours and should be understood as acting on high-level features rather than purely on the raw data. However, estimating counterfactuals in image features \citep{Pawlowski,Sanchez2022diffscm}, for example, requires invertible mechanisms such as normalizing flows \citep{papamakarios2019normalizing} and/or methods for variational inference \citep{Kingma2014} which have their own complexities. Another open problem is how to deal with multimodal data  e.g. images, text, age, sex and genetic data in a healthcare scenario as detailed in section \ref{sec:dimension_modal}.




